Mapping the magnetic field using a magnetometer array with noisy input Gaussian process regression

Ferromagnetic materials in indoor environments give rise to disturbances in the ambient magnetic field. Maps of these magnetic disturbances can be used for indoor localisation. A Gaussian process can be used to learn the spatially varying magnitude of the magnetic field using magnetometer measurements and information about the position of the magnetometer. The position of the magnetometer, however, is frequently only approximately known. This negatively affects the quality of the magnetic field map. In this paper, we investigate how an array of magnetometers can be used to improve the quality of the magnetic field map. The position of the array is approximately known, but the relative locations of the magnetometers on the array are known. We include this information in a novel method to make a map of the ambient magnetic field. We study the properties of our method in simulation and show that our method improves the map quality. We also demonstrate the efficacy of our method with experimental data for the mapping of the magnetic field using an array of 30 magnetometers.

==> Chapters/Backups.tex <==

\section{Our method}
We first show how the NIGP \cite{mchutchon2011gaussian} formulation was derived. Afterwards, we show how we can adapt the NIGP formulation to work with correlated inputs, in particular, we assume that input locations are placed on an array.
\subsection{Noisy input GPs}
We will now consider input locations to be noisy, introducing the term $\e_x$. The GP formulation changes to
\begin{equation}
    y_i = f(\x_i + \e_x) + e_y, \quad e_x \sim \N(0, \Sigma_x).
\end{equation}
The NIGP method was derived by taking the first-order Taylor expansion around the uncertain input locations resulting in the approximation:
\begin{equation}
    y_i \approx f(\x_i) + \e^T_x \frac{\partial f(\x_i)}{\partial \x_i} + e_y.
\end{equation}
This introduces an additional term 
\begin{equation}
    \bar{\Sigma}(x) =\frac{\partial f(\x_i)}{\partial \x_i}^T \Sigma_x \frac{\partial f(\x_i)}{\partial \x_i}
\end{equation}
which is treated as heteroskedastic output noise. This term includes the input uncertainty and the GP posterior gradient, which brings inherent structure from the data into the GP: Where our measurements are changing values rapidly over a small input space change (i.e. high gradient) this term brings larger uncertainties. Similarly, it adds little uncertainty where we have small gradients. By adding the additional term, we alleviate regular GP from overfitting where we have input uncertainties and rapidly changing outputs (i.e. high gradient values). As the derivative of a GP is also a GP, We can find the derivative to our latent function from the posterior. First, we introduce the derivative of the squared exponential kernel as
\begin{equation}
     \frac{\partial k(\x_i, \x_j)}{\partial \x_i} = -\left(\x_i - \x_j \right)\frac{\sigma_f^2}{l^2}  \exp{\left( - \frac{||\x_i-\x_j||^2}{2 l^2} \right)}.
\end{equation}
Then we can find the posterior gradient at any location $x_i$ as
\begin{equation}
    \nabla f(\x_i) = \nabla \K_i^T (\K + \sigma^2_y \I_n  )^{-1} y_i,
\end{equation}
Where the term $\nabla f(\x_i): \R^d \rightarrow \R^d$ is defined as
\begin{equation}
\nabla f(\x_i) = \begin{bmatrix}
    \frac{\partial f(\x_i)}{\partial x_{i_1}} & \hdots & \frac{\partial f(\x_i)}{\partial x_{i_d}}
\end{bmatrix}^T.
\end{equation}
We will make use of shorthand notation $ \nabla f_i = \nabla f(\x_i)$. The additional term in NIGP for more input locations stacks block-diagonally as
\begin{equation}
    \bar{\Sigma}_x(X) = 
    \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}^T
    \begin{bmatrix}
    \Sigma_x &  0 \\
    0 & \Sigma_x 
    \end{bmatrix}
      \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}.
\end{equation}
With this additional term, the GP posterior mean and covariance become
\begin{equation}
\begin{aligned}
    \bar{\f}_* &\sim \N(\bar{\mu}_*, \bar{\Sigma}_{**}), \\
    \bar{\mu}_* &= \K^T_* \left(  \K + \sigma^2_y \I_n + \bar{\Sigma}_x(X)  \right)^{-1} \y, \\
    \bar{\Sigma}_{**} &= \K_{**} - \K^T_* \left(  \K + \sigma^2_y \I_n  + \bar{\Sigma}_x(X) \right)^{-1} \K_* + \bar{\Sigma}_x(X_*).
    \label{eq:NIGP}
\end{aligned}
\end{equation}
The input noise is propagated via the derivative and acts as an additional output noise term. Note that the final term will only appear if we assume noisy predictive inputs. If we assume deterministic predictive inputs, this term is zero.  

\subsection{Correlated inputs}
Previously, every input location was considered independent. We place multiple sensors on an array, introducing rigid-body constraints. This creates correlations between input locations. In the form of an array, the joint covariance can be written as $H \Sigma_x H^T$. The added term from NIGP now changes to $ \widetilde{\Sigma}_x(X)$, where the input covariance is now correlated. The case we consider is an array of 2 inputs, which gives the correlated input covariance as
\begin{equation}
    \bar{\Sigma}_x(X) = 
    \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}^T
    \begin{bmatrix}
    \Sigma_x & \Sigma_x \\
    \Sigma_x & \Sigma_x 
    \end{bmatrix}
      \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}
\end{equation}
we scale this to more correlated input locations, they will then appear block-diagonally in the input covariance matrix. We now have the resulting posterior:
\begin{equation}
\begin{aligned}
    \widetilde{\f}_* &\sim \N(\widetilde{\mu}_*, \widetilde{\Sigma}_{**}), \\
    \widetilde{\mu}_* &= \K^T_* \left(  \K + \sigma^2_y \I_n   + \widetilde{\Sigma}_x(X) \right)^{-1} \y, \\
    \widetilde{\Sigma}_{**} &= \K_{**} - \K^T_* \left(  \K + \sigma^2_y \I_n  + \widetilde{\Sigma}_x(X) \right)^{-1} \K_* + \widetilde{\Sigma}_x(X_*).
    \label{eq:ArrayPosterior}
\end{aligned}
\end{equation}
Depending on the type of prediction, we can take either the correlated formulation or the NIGP formulation. We consider neither, and will assume deterministic training locations from now on, this will drop the last term in \eqref{eq:ArrayPosterior}.
\subsection{Comparison to NIGP}
The difference between our method and NIGP is in the joint input noise covariance structure. We will demonstrate the similarities and differences using an array of 2 sensors with the scalar input and output pairs $\{x_i, y_i\}_{i = 1}^2$ . For the array, the sensors are correlated by $H$ as $ \tilde{\x}_{1:2} = H\x, $
Where NIGP only takes diagonal entries, we have correlated input noise as seen in \eqref{} and \eqref{}. \color{red} dit eerder zeggen
\color{black}
It is easy to observe that if all derivatives are zero, they are equivalent to a normal GP regression without input noise. Secondly, if there is only one non-zero derivative, the two matrices are identical. This results in 
\begin{subequations}
\begin{align}
    & \begin{bmatrix} 
    \nabla f_1 & 0  \\
    0  & 0
    \end{bmatrix}
    \begin{bmatrix} 
    \Sigma_{x} & 0  \\
    0 & \Sigma_{x} 
    \end{bmatrix}
    \begin{bmatrix} 
    \nabla f_1 & 0  \\
    0  & 0
    \end{bmatrix} = \begin{bmatrix} 
    \nabla f_1 \Sigma_{x} \nabla f_1 & 0  \\
    0 & 0 
    \end{bmatrix},  \\
    & \begin{bmatrix} 
    \nabla f_1 & 0  \\
    0  & 0
    \end{bmatrix}
    \begin{bmatrix}
    \Sigma_{x} & \Sigma_{x}  \\
    \Sigma_{x} & \Sigma_{x} 
    \end{bmatrix}
    \begin{bmatrix} 
    \nabla f_1 & 0  \\
    0  & 0
    \end{bmatrix} = \begin{bmatrix} 
    \nabla f_1 \Sigma_{x} \nabla f_1 & 0  \\
    0 & 0 
    \end{bmatrix}
\end{align}
\end{subequations}
For further analysis, we will assume a constant gradient, i.e. $\nabla f_i = \nabla f_j$ and work out the terms in \eqref{eq:ArrayPosterior}. We abbreviate the term $ \nabla f_i \Sigma_{x} \nabla f_j$ to $\beta$ and show how our method differs from NIGP with the posterior mean 
\begin{subequations}
\begin{align}
    \mu^N_* &=  \frac{N_\E}{D_\E}, \\
    \mu^A_* &= \frac{N_\E - (k_{*1} \beta y_2 + k_{*2} \beta y_1 )}{D_\E - (k_{12} \beta + k_{21}\beta + \beta^2 ) },
\end{align}
\end{subequations}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/MeanComparison.pdf}
    \caption{Ook normal GP regression toevoegen?}
    \label{fig:MeanComparison}
\end{figure}
TODO: verhaaltje over wat we zien.
If we look at the two different posterior covariances, 
\begin{subequations}
\begin{align}
    \Sigma^N_{**} &=  k_{**} - \frac{N_\V}{D_\V}, \\
    \Sigma^A_{**} &=  k_{**} - \frac{N_\V - (k_{1*} \beta k_{2*} + k_{2*} \beta k_{1*})}{D_\V - (k_{12}\beta + k_{21}\beta + \beta^2 ) },
\end{align}
\end{subequations}
we see that three outcomes are possible. Namely, the posterior covariances are equal, one is larger or one is smaller than the other. This depends on the additional terms introduced by our method. 
\begin{equation}
    k_{2*} k_{1*}= \frac{k_{12} + k_{21} + \beta}{2}
    \label{eq:VarianceComparison}
\end{equation}
If the LHS in \eqref{eq:VarianceComparison} is bigger than the RHS, our method has bigger variance than NIGP, similarly, if the LHS is smaller than the RHS, we have smaller variance than NIGP. Finally, the two methods are equal when the LHS is equal to the RHS. This behaviour is shown in Fig. \ref{fig:VarianceComparison}. It shows that our method has a lower predictive variance around the collected data, however, as we get close to the data, we have higher variance. From \eqref{eq:VarianceComparison} we see that the product of the two prediction kernel elements is bigger than the RHS. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/VarianceComparison.pdf}
    \caption{Caption}
    \label{fig:VarianceComparison}
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/VarianceComparisonBig.pdf}
    \caption{Caption}
    \label{fig:VarianceComparisonBig}
\end{figure}

In Fig.\ref{fig:VarianceComparison} and Fig. \ref{fig:VarianceComparisonBig} we see how the variance of the prediction locations changes for our method compared to NIGP. Surrounding the array, our method has a lower variance w.r.t. NIGP. The interpretation of this is that we have added more information to the GP prior covariance. Interestingly, however, we see that if we have a sufficiently small array, the predictive variance of our method becomes larger than NIGP. The interpretation to this is that even though we have added more information, the location of the array is unknown. When the sensors are placed closely together, they provide (almost?) the same measurements, whereas as they are placed farther away, will differ in their measurement. \color{red} Checken of dit te maken heef tmet de lenght-scale? Waarschinlijk wel \color{black}



\section{}

For simplification, we assume a constant gradient, i.e. $\nabla f_i = \nabla f_j$ and work out the terms in \eqref{eq:ArrayPosterior}. We abbreviate the term $ \nabla f_i \Sigma_{x} \nabla f_j$ to $\beta$. In the equation below, $\bar{\mu}_*$ denotes the predictive mean of NIGP and $ \widetilde{\mu}_*$ denotes the predictive mean of our method.
\begin{subequations}
\begin{align}
    \bar{\mu}_* &= \K^T_* \left(  \K + \sigma^2_y \I_n   + \Sigma_x(X) \right)^{-1} \y = \frac{N_\E}{D_\E}, \\
    \widetilde{\mu}_* &= \frac{N_\E - (k_{*1} \beta y_2 + k_{*2} \beta y_1 )}{D_\E - (k_{12} \beta + k_{21}\beta + \beta^2 ) },
\end{align}
\end{subequations}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/MeanComparison.pdf}
    \caption{Ook normal GP regression toevoegen?}
    \label{fig:MeanComparison}
\end{figure}
TODO: verhaaltje over wat we zien.



\section{}

To compare our method against NIGP and a normal GP we run a Monte Carlo (MC) simulation with 100 runs. We use the squared exponential kernel with known hyper-parameters $\theta = \{l^2 = 1, \sigma_f^2 = 1, \sigma^2_y = 0.01\}$. We sample a random function from our GP prior for every MC simulation. We use the following parameters for every MC simulation. We place 5 sensors on the array, with an array size of 2. We use 10 array locations, for a total of 50 data points. We iterate once through \color{red} ref to chicken egg problem \color{black}. The input space lives in the domain of $ X \in \{-10, 10 \}$. We take an input error of $\Sigma_x = 0.25$. 
With the MC simulation, we will analyze the effects of varying the array size, the input error and \color{red} todo \color{black}. 


\subsection{Temporary placeholder, rewrite this subsection}

The size the of the array will influence on the posterior mean and the posterior variance. To show this, we look back at \eqref{eq:CorrelatedUncertainty}, where we show input noise covariance, so that we can analyze how the correlated input locations differ form NIGP. for clarity, we restate it here:
If we look at the two different posterior covariances, 
\begin{subequations}
\begin{align}
    \Sigma^N_{**} &=  k_{**} - \frac{N_\V}{D_\V}, \\
    \Sigma^A_{**} &=  k_{**} - \frac{N_\V - (k_{1*} \beta k_{2*} + k_{2*} \beta k_{1*})}{D_\V - (k_{12}\beta + k_{21}\beta + \beta^2 ) },
\end{align}
\end{subequations}
we see that three outcomes are possible. Namely, the posterior covariances are equal, one is larger or one is smaller than the other. This depends on the additional terms introduced by our method. 
\begin{equation}
    k_{2*} k_{1*}= \frac{k_{12} + k_{21} + \beta}{2}
    \label{eq:VarianceComparison}
\end{equation}
If the LHS in \eqref{eq:VarianceComparison} is bigger than the RHS, our method has bigger variance than NIGP, similarly, if the LHS is smaller than the RHS, we have smaller variance than NIGP. Finally, the two methods are equal when the LHS is equal to the RHS. This behaviour is shown in Fig. \ref{fig:VarianceComparison}. It shows that our method has a lower predictive variance around the collected data, however, as we get close to the data, we have higher variance. From \eqref{eq:VarianceComparison} we see that the product of the two prediction kernel elements is bigger than the RHS. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/VarianceComparison.pdf}
    \caption{Caption}
    \label{fig:VarianceComparison}
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/VarianceComparisonBig.pdf}
    \caption{Caption}
    \label{fig:VarianceComparisonBig}
\end{figure}

In Fig.\ref{fig:VarianceComparison} and Fig. \ref{fig:VarianceComparisonBig} we see how the variance of the prediction locations changes for our method compared to NIGP. Surrounding the array, our method has a lower variance w.r.t. NIGP. The interpretation of this is that we have added more information to the GP prior covariance. Interestingly, however, we see that if we have a sufficiently small array, the predictive variance of our method becomes larger than NIGP. The interpretation to this is that even though we have added more information, the location of the array is unknown. When the sensors are placed closely together, they provide (almost?) the same measurements, whereas as they are placed farther away, will differ in their measurement. 



the posterior mean function if flat and Algorithm-1 and NIGP are identical to a regular GP from \eqref{eq:GPposterior}. If only one 

Another interesting case is observed when only one 

(i.e. $\nabla f(\x_i) \neq 0, \nabla f(\x_j) = 0,  j = 1,\dots, N, j \neq i$
%(i.e. $\nabla f(\x_1) \neq 0, \nabla f(\x_{2:N}) = 0$)

only gets propogated to the output if there is enough spatial variaton in the data.
For Algorithm~1 to take the input uncertainty into account, there must be enough spatial variation in the data. To illustrate, we consider two sensors on an array, and look at the additional input covariance noise term $\Sigma(X^\text{n}_{1:k})$
\begin{equation*}
\begin{aligned}
    \Sigma(\widetilde{X}_i) &= \frac{\partial f(\widetilde{X}_i)}{\partial \widetilde{X}_i}^T \left( H \Sigma_x H^T \right) \frac{\partial f(\widetilde{X}_i)}{\partial \widetilde{X}_i}, \\
    &= 
    \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}^T
    \begin{bmatrix}
    \Sigma_x & \Sigma_x \\
    \Sigma_x & \Sigma_x 
    \end{bmatrix}
      \begin{bmatrix}
    \nabla f_1 & 0 \\
    0 & \nabla f_2 
    \end{bmatrix}.
\end{aligned}
\end{equation*}
where we make use of shorthand notation $ \nabla f_i = \nabla f(\x_i)$. If the posterior function is flat (i.e. $\nabla f_1 = \nabla f_2 = 0$), our method is equal to regular GP from \eqref{eq:GPposterior}. Secondly, if there is only one non-zero derivative (i.e., only one sensor lies on a gradient, and the other sensor lies on a flat part of the function), the two matrices are identical. Thirdly, the joint covariance structure that arises from $H \Sigma_x H^T$, tells us that where NIGP treats each data point independently, our method treats the error of the array as a single input error. This has two effects: first, Algorithm~1 can capture the spatial variation of the latent function $\f$ between the sensors on the array. Second, we anticipate a reduction in the posterior variance for our method.


\begin{table}[h]
\caption{Average RMSE and its standard deviation of 50 downsampled data sets with 2400 data points. TODO change to plot with more covariances}
\begin{center}
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{\textbf{Average RMSE $ [-] \times 10^{-2}$}}
 \\
\hline
 &\multicolumn{3}{c}{\textbf{Dataset 1}}  
 \\
  & \textbf{$\Sigma^{(1)}_x $}& \textbf{$\Sigma^{(2)}_x $}& \textbf{$\Sigma^{(3)}_x $}\\
\hline
GP & 1.90 $\pm$ 0.26  & 3.27 $\pm$ 0.42 & 4.14 $\pm$ 0.52 \\
NIGP & 1.87 $\pm$ 0.27 & 3.17 $\pm$ 0.39 & 3.94  $\pm$ 0.41  \\
Algorithm~1 & 1.63 $\pm$ 0.23 & 2.77 $\pm$ 0.31 & 3.72  $\pm$ 0.41 \\
\hline
& \multicolumn{3}{c}{\textbf{Dataset 2}} \\
 & \textbf{$\Sigma^{(1)}_x$}& \textbf{$\Sigma^{(2)}_x $}& \textbf{$\Sigma^{(3)}_x $} \\
\hline
GP & 2.67 $\pm$ 0.57 & 4.50 $\pm$ 1.14 & 6.05 $\pm$ 1.80 \\
NIGP & 2.54  $\pm$ 0.54 & 3.83 $\pm$ 0.91 & 4.79 $\pm$ 1.30 \\
Algorithm~1 & 1.99  $\pm$ 0.48 & 3.04 $\pm$ 0.78 & 4.31 $\pm$ 1.31 \\
\end{tabular}
\label{tab:MagnetometerArrayRSME}
\end{center}
\end{table}


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

